Structured Residual Dynamics Augmented Predictive Control for Indirect Drone-Ball Manipulation

Indirect drone-ball manipulation requires controlling a freely rolling ball through drone-driven beam motion. This paper presents a nonlinear model predictive control (NMPC) framework for time-varying ball trajectory tracking. The nominal ball-beam dynamics are augmented by a first-order model of the drone velocity response with command dead time. A structured ball-acceleration residual is further introduced, motivated by position-dependent and dissipative patterns in the model mismatch. The resulting dynamics are used in both a state predictor for delay compensation and NMPC. Using the nominal dynamics, NMPC outperforms a nonlinear feedforward-feedback controller in simulation. Adding the structured residual to the nominal dynamics improves multi-step prediction on held-out real-world data. In physical experiments, NMPC using the residual-augmented dynamics reduces overall steady-state error in constant-reference balancing by 50.7% and mean absolute error in dynamic tracking by 37.2% relative to NMPC using the nominal dynamics. Although the model augmented with a multilayer perceptron (MLP) residual achieves lower offline prediction errors, NMPC using the structured residual achieves better overall closed-loop accuracy and more reliable execution than NMPC using the MLP residual.

==> tables/distribution_revision/numbers.tex <==
% Generated from unchanged archived distribution results.
\newcommand{\DistRevTrials}{54}
\newcommand{\DistRevCompleted}{48}
\newcommand{\DistRevTerminated}{6}
\newcommand{\DistRevTrainingTrials}{79}
\newcommand{\DistRevValidationTrials}{6}
\newcommand{\DistRevTestTrials}{6}
\newcommand{\DistRevOctoberDynamicQ}{5.5}
\newcommand{\DistRevSeptemberDynamicQ}{20.7}
\newcommand{\DistRevTerminatedQ}{51.3}
\newcommand{\DistRevPhysicalMaxGap}{0.66}
\newcommand{\DistRevValidationQ}{1.0}
\newcommand{\DistRevTestQ}{2.6}
\newcommand{\DistRevConstantQ}{15.0}
\newcommand{\DistRevDynamicQ}{18.2}


==> tables/equilibrium_revision/numbers.tex <==
% Generated from results/equilibrium_revision; do not edit numerical values.
\newcommand{\EqRevLooseMLPTrials}{13}
\newcommand{\EqRevLooseMLPWindows}{73}
\newcommand{\EqRevLooseStructuredTrials}{18}
\newcommand{\EqRevLooseStructuredWindows}{118}
\newcommand{\EqRevMLPTrials}{9}
\newcommand{\EqRevMLPWindows}{38}
\newcommand{\EqRevStallTrials}{8}
\newcommand{\EqRevStallWindows}{30}
\newcommand{\EqRevStructuredTrials}{15}
\newcommand{\EqRevStructuredWindows}{58}
\newcommand{\EqRevStrictMLPTrials}{5}
\newcommand{\EqRevStrictMLPWindows}{16}
\newcommand{\EqRevStrictStructuredTrials}{5}
\newcommand{\EqRevStrictStructuredWindows}{11}
\newcommand{\EqRevMLPMLPAngleMean}{0.613}
\newcommand{\EqRevMLPMLPAngleSD}{0.487}
\newcommand{\EqRevMLPMLPAccelMean}{0.0544}
\newcommand{\EqRevMLPMLPAccelSD}{0.0428}
\newcommand{\EqRevMLPMLPStaticMean}{0.0534}
\newcommand{\EqRevMLPMLPStaticSD}{0.0402}
\newcommand{\EqRevMLPMLPTowardPctMean}{88.9}
\newcommand{\EqRevMLPMLPTowardPctSD}{33.3}
\newcommand{\EqRevMLPMLPAlignedBiasMean}{0.0424}
\newcommand{\EqRevMLPMLPAlignedBiasSD}{0.0561}
\newcommand{\EqRevMLPMLPAlignedPredictionMean}{0.0411}
\newcommand{\EqRevMLPMLPAlignedPredictionSD}{0.0551}
\newcommand{\EqRevMLPMLPMAEMean}{13.71}
\newcommand{\EqRevMLPMLPMAESD}{9.16}
\newcommand{\EqRevMLPMLPCommandSpanMean}{0.159}
\newcommand{\EqRevMLPMLPCommandSpanSD}{0.052}
\newcommand{\EqRevMLPMLPIncrementMean}{0.022}
\newcommand{\EqRevMLPMLPIncrementSD}{0.017}
\newcommand{\EqRevMLPNominalAngleMean}{0.510}
\newcommand{\EqRevMLPNominalAngleSD}{0.319}
\newcommand{\EqRevMLPNominalAccelMean}{0.0629}
\newcommand{\EqRevMLPNominalAccelSD}{0.0403}
\newcommand{\EqRevMLPNominalStaticMean}{0.0624}
\newcommand{\EqRevMLPNominalStaticSD}{0.0390}
\newcommand{\EqRevMLPNominalTowardPctMean}{42.6}
\newcommand{\EqRevMLPNominalTowardPctSD}{50.8}
\newcommand{\EqRevMLPNominalAlignedBiasMean}{0.0019}
\newcommand{\EqRevMLPNominalAlignedBiasSD}{0.0764}
\newcommand{\EqRevMLPNominalAlignedPredictionMean}{0.0007}
\newcommand{\EqRevMLPNominalAlignedPredictionSD}{0.0744}
\newcommand{\EqRevMLPNominalMAEMean}{13.71}
\newcommand{\EqRevMLPNominalMAESD}{9.16}
\newcommand{\EqRevMLPNominalCommandSpanMean}{0.159}
\newcommand{\EqRevMLPNominalCommandSpanSD}{0.052}
\newcommand{\EqRevMLPNominalIncrementMean}{0.022}
\newcommand{\EqRevMLPNominalIncrementSD}{0.017}
\newcommand{\EqRevMLPStructuredAngleMean}{0.589}
\newcommand{\EqRevMLPStructuredAngleSD}{0.410}
\newcommand{\EqRevMLPStructuredAccelMean}{0.0720}
\newcommand{\EqRevMLPStructuredAccelSD}{0.0514}
\newcommand{\EqRevMLPStructuredStaticMean}{0.0720}
\newcommand{\EqRevMLPStructuredStaticSD}{0.0502}
\newcommand{\EqRevMLPStructuredTowardPctMean}{75.9}
\newcommand{\EqRevMLPStructuredTowardPctSD}{43.4}
\newcommand{\EqRevMLPStructuredAlignedBiasMean}{0.0469}
\newcommand{\EqRevMLPStructuredAlignedBiasSD}{0.0762}
\newcommand{\EqRevMLPStructuredAlignedPredictionMean}{0.0457}
\newcommand{\EqRevMLPStructuredAlignedPredictionSD}{0.0755}
\newcommand{\EqRevMLPStructuredMAEMean}{13.71}
\newcommand{\EqRevMLPStructuredMAESD}{9.16}
\newcommand{\EqRevMLPStructuredCommandSpanMean}{0.159}
\newcommand{\EqRevMLPStructuredCommandSpanSD}{0.052}
\newcommand{\EqRevMLPStructuredIncrementMean}{0.022}
\newcommand{\EqRevMLPStructuredIncrementSD}{0.017}
\newcommand{\EqRevStructuredMLPAngleMean}{0.299}
\newcommand{\EqRevStructuredMLPAngleSD}{0.185}
\newcommand{\EqRevStructuredMLPAccelMean}{0.0282}
\newcommand{\EqRevStructuredMLPAccelSD}{0.0177}
\newcommand{\EqRevStructuredMLPStaticMean}{0.0275}
\newcommand{\EqRevStructuredMLPStaticSD}{0.0176}
\newcommand{\EqRevStructuredMLPTowardPctMean}{75.8}
\newcommand{\EqRevStructuredMLPTowardPctSD}{40.9}
\newcommand{\EqRevStructuredMLPAlignedBiasMean}{0.0229}
\newcommand{\EqRevStructuredMLPAlignedBiasSD}{0.0245}
\newcommand{\EqRevStructuredMLPAlignedPredictionMean}{0.0229}
\newcommand{\EqRevStructuredMLPAlignedPredictionSD}{0.0238}
\newcommand{\EqRevStructuredMLPMAEMean}{2.03}
\newcommand{\EqRevStructuredMLPMAESD}{1.34}
\newcommand{\EqRevStructuredMLPCommandSpanMean}{0.221}
\newcommand{\EqRevStructuredMLPCommandSpanSD}{0.034}
\newcommand{\EqRevStructuredMLPIncrementMean}{0.023}
\newcommand{\EqRevStructuredMLPIncrementSD}{0.004}
\newcommand{\EqRevStructuredNominalAngleMean}{0.637}
\newcommand{\EqRevStructuredNominalAngleSD}{0.372}
\newcommand{\EqRevStructuredNominalAccelMean}{0.0777}
\newcommand{\EqRevStructuredNominalAccelSD}{0.0462}
\newcommand{\EqRevStructuredNominalStaticMean}{0.0779}
\newcommand{\EqRevStructuredNominalStaticSD}{0.0454}
\newcommand{\EqRevStructuredNominalTowardPctMean}{54.6}
\newcommand{\EqRevStructuredNominalTowardPctSD}{49.1}
\newcommand{\EqRevStructuredNominalAlignedBiasMean}{0.0336}
\newcommand{\EqRevStructuredNominalAlignedBiasSD}{0.0850}
\newcommand{\EqRevStructuredNominalAlignedPredictionMean}{0.0336}
\newcommand{\EqRevStructuredNominalAlignedPredictionSD}{0.0849}
\newcommand{\EqRevStructuredNominalMAEMean}{2.03}
\newcommand{\EqRevStructuredNominalMAESD}{1.34}
\newcommand{\EqRevStructuredNominalCommandSpanMean}{0.221}
\newcommand{\EqRevStructuredNominalCommandSpanSD}{0.034}
\newcommand{\EqRevStructuredNominalIncrementMean}{0.023}
\newcommand{\EqRevStructuredNominalIncrementSD}{0.004}
\newcommand{\EqRevStructuredStructuredAngleMean}{0.328}
\newcommand{\EqRevStructuredStructuredAngleSD}{0.276}
\newcommand{\EqRevStructuredStructuredAccelMean}{0.0407}
\newcommand{\EqRevStructuredStructuredAccelSD}{0.0340}
\newcommand{\EqRevStructuredStructuredStaticMean}{0.0401}
\newcommand{\EqRevStructuredStructuredStaticSD}{0.0337}
\newcommand{\EqRevStructuredStructuredTowardPctMean}{89.0}
\newcommand{\EqRevStructuredStructuredTowardPctSD}{20.5}
\newcommand{\EqRevStructuredStructuredAlignedBiasMean}{0.0389}
\newcommand{\EqRevStructuredStructuredAlignedBiasSD}{0.0358}
\newcommand{\EqRevStructuredStructuredAlignedPredictionMean}{0.0389}
\newcommand{\EqRevStructuredStructuredAlignedPredictionSD}{0.0354}
\newcommand{\EqRevStructuredStructuredMAEMean}{2.03}
\newcommand{\EqRevStructuredStructuredMAESD}{1.34}
\newcommand{\EqRevStructuredStructuredCommandSpanMean}{0.221}
\newcommand{\EqRevStructuredStructuredCommandSpanSD}{0.034}
\newcommand{\EqRevStructuredStructuredIncrementMean}{0.023}
\newcommand{\EqRevStructuredStructuredIncrementSD}{0.004}
\newcommand{\EqRevStallMLPAngleMean}{0.635}
\newcommand{\EqRevStallMLPAngleSD}{0.516}
\newcommand{\EqRevStallMLPAccelMean}{0.0558}
\newcommand{\EqRevStallMLPAccelSD}{0.0456}
\newcommand{\EqRevStallMLPStaticMean}{0.0551}
\newcommand{\EqRevStallMLPStaticSD}{0.0426}
\newcommand{\EqRevStallMLPTowardPctMean}{87.5}
\newcommand{\EqRevStallMLPTowardPctSD}{35.4}
\newcommand{\EqRevStallMLPAlignedBiasMean}{0.0422}
\newcommand{\EqRevStallMLPAlignedBiasSD}{0.0600}
\newcommand{\EqRevStallMLPAlignedPredictionMean}{0.0408}
\newcommand{\EqRevStallMLPAlignedPredictionSD}{0.0589}
\newcommand{\EqRevStallMLPMAEMean}{15.01}
\newcommand{\EqRevStallMLPMAESD}{8.92}
\newcommand{\EqRevStallMLPCommandSpanMean}{0.161}
\newcommand{\EqRevStallMLPCommandSpanSD}{0.055}
\newcommand{\EqRevStallMLPIncrementMean}{0.023}
\newcommand{\EqRevStallMLPIncrementSD}{0.018}
\newcommand{\EqRevStallNominalAngleMean}{0.548}
\newcommand{\EqRevStallNominalAngleSD}{0.319}
\newcommand{\EqRevStallNominalAccelMean}{0.0677}
\newcommand{\EqRevStallNominalAccelSD}{0.0403}
\newcommand{\EqRevStallNominalStaticMean}{0.0670}
\newcommand{\EqRevStallNominalStaticSD}{0.0390}
\newcommand{\EqRevStallNominalTowardPctMean}{47.9}
\newcommand{\EqRevStallNominalTowardPctSD}{51.5}
\newcommand{\EqRevStallNominalAlignedBiasMean}{0.0053}
\newcommand{\EqRevStallNominalAlignedBiasSD}{0.0809}
\newcommand{\EqRevStallNominalAlignedPredictionMean}{0.0039}
\newcommand{\EqRevStallNominalAlignedPredictionSD}{0.0789}
\newcommand{\EqRevStallNominalMAEMean}{15.01}
\newcommand{\EqRevStallNominalMAESD}{8.92}
\newcommand{\EqRevStallNominalCommandSpanMean}{0.161}
\newcommand{\EqRevStallNominalCommandSpanSD}{0.055}
\newcommand{\EqRevStallNominalIncrementMean}{0.023}
\newcommand{\EqRevStallNominalIncrementSD}{0.018}
\newcommand{\EqRevStallStructuredAngleMean}{0.612}
\newcommand{\EqRevStallStructuredAngleSD}{0.436}
\newcommand{\EqRevStallStructuredAccelMean}{0.0747}
\newcommand{\EqRevStallStructuredAccelSD}{0.0547}
\newcommand{\EqRevStallStructuredStaticMean}{0.0748}
\newcommand{\EqRevStallStructuredStaticSD}{0.0533}
\newcommand{\EqRevStallStructuredTowardPctMean}{72.9}
\newcommand{\EqRevStallStructuredTowardPctSD}{45.4}
\newcommand{\EqRevStallStructuredAlignedBiasMean}{0.0465}
\newcommand{\EqRevStallStructuredAlignedBiasSD}{0.0817}
\newcommand{\EqRevStallStructuredAlignedPredictionMean}{0.0451}
\newcommand{\EqRevStallStructuredAlignedPredictionSD}{0.0810}
\newcommand{\EqRevStallStructuredMAEMean}{15.01}
\newcommand{\EqRevStallStructuredMAESD}{8.92}
\newcommand{\EqRevStallStructuredCommandSpanMean}{0.161}
\newcommand{\EqRevStallStructuredCommandSpanSD}{0.055}
\newcommand{\EqRevStallStructuredIncrementMean}{0.023}
\newcommand{\EqRevStallStructuredIncrementSD}{0.018}


==> tables/numbers.tex <==
% Generated; see results/document_numbers.json for provenance.
\newcommand{\SolverAttempts}{14}
\newcommand{\SolverCompleted}{11}
\newcommand{\ReferenceCount}{223}
\newcommand{\ReferenceAccepted}{216}
\newcommand{\ReferenceFailed}{7}
\newcommand{\RegularReferenceCount}{200}
\newcommand{\RegularReferenceAccepted}{198}
\newcommand{\EventReferenceCount}{23}
\newcommand{\EventReferenceAccepted}{18}
\newcommand{\LThreeActionRelative}{58.79}
\newcommand{\LThreeActionError}{0.04899}
\newcommand{\LThreeMAE}{21.24}
\newcommand{\LThreePosition}{0.338}
\newcommand{\LNineActionRelative}{3.67}
\newcommand{\LNineActionError}{0.00306}
\newcommand{\LNineMAE}{24.24}
\newcommand{\LNinePosition}{0.592}
\newcommand{\TrainingTrials}{79}
\newcommand{\TrainingPoints}{139802}
\newcommand{\NormalizationPoints}{139811}
\newcommand{\HistoricalTrials}{54}
\newcommand{\HistoricalCompleted}{48}
\newcommand{\ObservationJumps}{12}
\newcommand{\NonfiniteExcluded}{0}
\newcommand{\CoverageThreshold}{0.563879}
\newcommand{\PhysicalThreshold}{0.529293}
\newcommand{\PcaTwoVariance}{70.76}
\newcommand{\PcaFourVariance}{99.95}
\newcommand{\SupportCounterexampleCount}{13}
\newcommand{\HTwoMAE}{35.83}
\newcommand{\HFiveMAE}{39.14}
\newcommand{\HTwentyFourMAE}{9.71}
\newcommand{\HTwentyNineMAE}{9.61}
\newcommand{\HThirteenExceed}{95.28}
\newcommand{\HEighteenExceed}{99.22}
\newcommand{\LowSpeedTrialCount}{17}
\newcommand{\HSeventeenPosition}{0.200}
\newcommand{\HSeventeenMLPAcceleration}{0.152}
\newcommand{\HSeventeenStructuredAcceleration}{0.189}
\newcommand{\HSeventeenNominalAcceleration}{0.142}
\newcommand{\HSeventeenDroneRMS}{0.036}
\newcommand{\LowSpeedFractionMean}{50.6}
\newcommand{\EquilibriumCommand}{0.00485}
\newcommand{\SolverObservationJumps}{20}


==> tables/solver_revision/numbers.tex <==
% Generated from results/solver_revision/document_numbers.json
\newcommand{\RevBaselineSnapshots}{156}
\newcommand{\RevBaselineTrials}{54}
\newcommand{\RevBaselineConverged}{81}
\newcommand{\RevBaselineNonconverged}{75}
\newcommand{\RevBaselineNonconvergedTrials}{40}
\newcommand{\RevBaselinePeriodTwo}{50}
\newcommand{\RevBaselinePeriodTwoTrials}{32}
\newcommand{\RevBaselineBudget}{75}
\newcommand{\RevBaselineAbnormal}{0}
\newcommand{\RevBaselineReferenceAccepted}{154}
\newcommand{\RevRTIConvergedTrials}{38}
\newcommand{\RevRTIConvergedMeanUpdates}{19.7}
\newcommand{\RevRTIConvergedMeanGap}{0.00430}
\newcommand{\RevRTIConvergedSDGap}{0.00640}
\newcommand{\RevReplayMax}{0.167}
\newcommand{\RevReplayMedianMax}{0.167}
\newcommand{\RevPredictorError}{2.22e-16}
\newcommand{\RevPreviewError}{1.27e-13}
\newcommand{\RevOriginalConstantMAE}{25.92}
\newcommand{\RevOriginalConstantRun}{404}
\newcommand{\RevOriginalSineMAE}{13.03}
\newcommand{\RevOriginalSineRun}{94}
\newcommand{\RevGridOriginalMean}{0.03036}
\newcommand{\RevGridOriginalSD}{0.01864}
\newcommand{\RevGridOriginalWorst}{0.07054}
\newcommand{\RevGridOriginalRun}{126}
\newcommand{\RevGridOriginalInvalid}{0}
\newcommand{\RevGridOriginalPassed}{3}
\newcommand{\RevGridOriginalUpdates}{7.0}
\newcommand{\RevGridOriginalInitialPassed}{0}
\newcommand{\RevGridAMean}{0.00911}
\newcommand{\RevGridASD}{0.00453}
\newcommand{\RevGridAWorst}{0.01826}
\newcommand{\RevGridARun}{3}
\newcommand{\RevGridAInvalid}{0}
\newcommand{\RevGridAPassed}{10}
\newcommand{\RevGridAUpdates}{33.0}
\newcommand{\RevGridAInitialPassed}{0}
\newcommand{\RevGridBMean}{0.00389}
\newcommand{\RevGridBSD}{0.00201}
\newcommand{\RevGridBWorst}{0.00836}
\newcommand{\RevGridBRun}{2}
\newcommand{\RevGridBInvalid}{0}
\newcommand{\RevGridBPassed}{10}
\newcommand{\RevGridBUpdates}{26.0}
\newcommand{\RevGridBInitialPassed}{0}
\newcommand{\RevGridMainTrials}{9}
\newcommand{\RevGridDifficultStates}{12}
\newcommand{\RevGridMainSteps}{16203}
\newcommand{\RevGridReferences}{567}
\newcommand{\RevGridAcceptedReferences}{567}
\newcommand{\RevGridFailedReferences}{0}
\newcommand{\RevMAERTIConstant}{17.77}
\newcommand{\RevSERTI}{14.29}
\newcommand{\RevSERTISD}{9.82}
\newcommand{\RevMAERTISine}{13.68}
\newcommand{\RevRMSERTI}{16.50}
\newcommand{\RevRMSERTISD}{2.90}
\newcommand{\RevMAEAConstant}{17.51}
\newcommand{\RevSEA}{17.75}
\newcommand{\RevSEASD}{8.56}
\newcommand{\RevMAEASine}{7.66}
\newcommand{\RevRMSEA}{9.79}
\newcommand{\RevRMSEASD}{2.10}
\newcommand{\RevMAEBConstant}{15.95}
\newcommand{\RevSEB}{15.64}
\newcommand{\RevSEBSD}{8.03}
\newcommand{\RevMAEBSine}{9.85}
\newcommand{\RevRMSEB}{11.34}
\newcommand{\RevRMSEBSD}{-}
\newcommand{\RevOnlineDeadline}{12}

